Online TSP with Predictions

We initiate the study of online routing problems with predictions, inspired by recent exciting results in the area of learning-augmented algorithms. A learning-augmented online algorithm which incorporates predictions in a black-box manner to outperform existing algorithms if the predictions are accurate while otherwise maintaining theoretical guarantees even when the predictions are extremely erroneous is a popular framework for overcoming pessimistic worst-case competitive analysis. In this study, we particularly begin investigating the classical online traveling salesman problem (OLTSP), where future requests are augmented with predictions. Unlike the prediction models in other previous studies, each actual request in the OLTSP, associated with its arrival time and position, may not coincide with the predicted ones, which, as imagined, leads to a troublesome situation. Our main result is to study different prediction models and design algorithms to improve the best-known results in the different settings. Moreover, we generalize the proposed results to the online dial-a-ride problem.

==> Online TSP with Predictions_v1r/sec_1_intro.tex <==
\section{Introduction}
In many applications, people make decisions without knowing the future, and two approaches are widely used to address this issue: machine learning and online algorithms.
While machine learning methods usually lack theoretical guarantees, online algorithms are often evaluated based on the ratio of the optimal offline cost to the cost achieved by online algorithms over 
%%shou all 
worst-case
instances (i.e., the competitive ratio).
% the worst-case competitive ratio: we compare the optimal cost, denoted by $\costopt$, and the cost achieved by an algorithm, denoted by $\costalg$. 

In recent years, a rapidly growing field of research known as learning augmentation has attempted to 
%%shou
merge the above two approaches: 
incorporating machine-learned predictions into online algorithms 
%%shou
from a theoretical point of view. 
%%shou
In this line of work, such an algorithm is given some type of prediction 
%%shou related 
to the input, but the prediction is not always accurate. The goal of these studies is to design novel algorithms that have the following three properties: (1) achieve good performance when the 
%%shou provided 
given 
prediction is perfectly accurate, which is called {\it consistency}, (2) maintain worst-case bounds when the prediction is terribly wrong, which is called {\it robustness}, and (3) the performance should not degrade significantly when the prediction is slightly inaccurate, which is called {\it smoothness}. As the competitive ratio of a learning-augmented algorithm depends on errors, we define it as a function 
%%shou $c(.)$  c is better?
$c$
of error $\varepsilon$ using 
%%shou
a given predictor 
such that $c(\varepsilon)$ represents the worst-case competitive ratio given 
%%shou
that the error is at most $\varepsilon$. Note that the definition of $\varepsilon$ is subject to the problem setting (as shown in Section 2).
Optimization problems that have been studied under this framework include online paging \cite{jiang2020online, lykouris2021competitive, rohatgi2020nearoptimal, wei2020better}, ski-rental \cite{anand2020customizing, gollapudi2019online, kumar2018improving, wei2020optimal}, scheduling \cite{bamas2020learning, im2021nonclairvoyant, lattanzi2020online, kumar2018improving, wei2020optimal}, matching \cite{AGKK20}, bin packing \cite{angelopoulos2019online}, queueing \cite{mitzenmacher2021queues}, secretary \cite{AGKK20, dutting2021secretaries}, covering \cite{bamas2020primal}, bidding \cite{medina2017revenue}, knapsack \cite{im2021online}, facility location \cite{FGGP21}, and graph \cite{azar2022online} problems. 


However, 
%%shou except for 
in addition to 
the above online optimization problems, no existing studies extended the learning-augmented framework to 
%%shou the 
online routing problems, accompanied by many real-world applications. 
%%shou E.g. in recent years, 
For example, due to COVID-19, 
people have become more reliant on online food 
%%shou ordering 
delivery 
platforms such as Seamless 
%%shou or 
and 
Uber Eats. As a result, optimizing the delivery route 
%%shou has become 
is 
an important issue for the platform to win over such a huge market. 
Many platforms have used machine learning techniques to improve their 
%%shou products, 
services, 
but most studies did not provide worst-case guarantees. In this study, we look at how the learning-augmented framework can be applied to 
%%shou the 
online routing problems.
Note that 
%%shou some 
previous research in online learning also studied the combination of online algorithms and machine learning for routing problems; 
%%shou
readers may refer to the survey~\cite{blum1998online} for more details. 
%%
However, our study aims at designing a route with predictions which learned from historical 
%%shou data 
information rather than 
%%shou
choosing the best possible 
%%shou route 
strategy 
%%shou for 
adaptively 
based on some given routes. 
%%shou adaptively that is reported in \cite{blum1998online}.
%%
% which is the first step to bridge the gap between real-world applications and theoretical guarantees in the online routing problems. 
%%
%%shou Specifically, 
In particular, 
we study the online TSP problem proposed by Ausiello et.al.~\cite{ausiello2001algorithms} 
%%shou
and then extend to the 
%%shou related 
online dial-a-ride problem.



% We use the competitive ratio to measure the performance of an online algorithm. 
Let the offline optimal cost and the cost achieved by an online algorithm 
%%shou
be denoted by $\costopt$ and $\costalg$, respectively. 
% We say an online algorithm
%%
% \begin{definition}[Competitive Ratio]\label{def:CR}
% We say an online algorithm is $c$-competitive if there exists a constant $c$ such that $\costalg \leq c \cdot \costopt$ over any input instance.
% \end{definition}
%%
% Next, to 
To measure 
%%shou
the performance of an learning-augmented online algorithm, we follow the definitions proposed in \cite{lykouris2021competitive,kumar2018improving}. 

\begin{definition}[Consistency]\label{def:con}
An algorithm is said to be $\alpha$-consistent if $c(0)=\alpha$.
\end{definition}
\begin{definition}[Robustness]\label{def:rob}
An algorithm is said to be $\beta$-robust if $c(\varepsilon) \leq \beta$ for 
%%shou all 
any 
$\varepsilon$.
\end{definition}
\begin{definition}[Smoothness]\label{def:smo}
Given an $\alpha$-consistent algorithm, 
%0403 An algorithms 
it is said to be $f(\varepsilon)$-smooth if 
%0403 the cost of a learning-augmented algorithm is always bounded by 
$\costalg \leq \alpha \cdot \costopt + f(\varepsilon)$ holds on any input for some 
continuous
function $f$ such that $f(0) = 0$.
\end{definition}

%\medskip
\noindent{\textbf{The OLTSP.}}
In this study, we first consider one of the classical online combinatorial optimization problems, the online traveling salesman problem (OLTSP), in which the input is a sequence of requests that arrive 
%%shou serially. 
in an online fashion. 
A salesman, the server, is out to visit every request after it arrives and eventually return to the origin 
%%shou in an efficient way so 
such 
that the completion time is minimized. 
%%shou
Ausiello et.al.~\cite{ausiello2001algorithms} showed that the problem has a lower bound of 2 and presented 
an optimal 2-competitive algorithm, called \textsc{Plan-At-Home (PAH)}. 
Meanwhile, 
% With a sequence of improved results \cite{ausiello2004algorithms}, 
the currently best polynomial-time algorithm is approximately $2.65$-competitive~\cite{ascheuer2000online}. 

\medskip
\noindent{\textbf{The OLDARP.}}
We also consider the (uncapacitated) online dial-a-ride problem (OLDARP), which is a generalization of the OLTSP and has the same lower bound of 2. 
%%shou One of the main 
The key
difference between the two problems is that a server needs to transport each request from its 
%0416 source
pickup position
to its
%0403 corresponding destination
delivery position. 
%%shou We focus on the case where the server has unlimited capacity.
An optimal 
%%shou , which is 
$2$-competitive algorithm 
%%shou has been 
was
proposed in~\cite{ascheuer2000online}.

\medskip
%%shou
\noindent{\textbf{The OLTSP with Predictions.}}
The first 
%%shou step in 
question for
developing learning-augmented algorithms is: 
%%shou to ask: 
``what kind of predictions 
%%shou do we need 
are required
for the problem ?'' 
We refer to the discussion in \cite{lattanzi2020online} to answer this question: a good prediction should be learnable; that is, it should be possible to learn the prediction from historical data with an appropriate sample complexity. 
%%shou
For the OLTSP, 
it is natural to forecast its future requests.
To show the learnability, one can set up a learning task and   
%%shou use the 
exploit some 
different features 
of historical data, e.g., position of the requests, 
%%shou
arrival time of the requests, and the number of total requests,
%0416 etc... 
to learn a function; for instance, to minimize the mean square error (mse).
In this study, we 
%%shou
thus 
investigate three models with different types of predictions. 
%%shou
Notice that 
the significant difference between these predictions
is whether the 
%%shou historical data 
input
scale 
%%shou necessary 
is known 
for learning.
In the first two models, 
intuitively, we predict the whole sequence. 
%%shou and further consider two models.
%0407 while ignoring the computational issue
Formally, each request in the prediction has its 
%%shou
own predicted arrival time and position. 
%%
We split into two cases: \emph{the sequence prediction without identity} is a predicted sequence with an arbitrary size 
%%shou
over requests, and \emph{the sequence prediction with identity} is a predicted sequence that contains the exact same number of requests as the actual input. These two sequence predictions represent different learning models; the former one views the sequence of requests as a group, while the latter one examines each of the requests individually.
Last, we consider 
%%shou
a special prediction model, called 
\emph{the prediction of the last arrival time}, where the server receives the least amount of information %%shou among 
in 
the three models. The reason of choosing 
%%shou this 
such a 
prediction is that the arrival time of the last request actually provides a 
%0403 guess of the 
lower bound for the optimal route and that this information is enough to help the server in a polynomial setting. 
In the following sections, we show how to design learning-augmented online algorithms by 
%%shou coping with the 
%0403 pure 
%%shou 
appropriately incorporating 
the predictions into
online algorithms. 
As expected, predicting a sequence of requests provides more information about future events, 
%%shou 
certainly 
leading to a relatively higher cost than predicting a single request. 
%%shou 
That is, 
the choice of predictions can be read as a trade-off between the performance of online algorithms and the sample complexity.

\medskip
\noindent{\textbf{Our Contributions.}}
%%shou  Our main 
The key
contribution is to develop three models for the OLTSP in each of which we present a learning-augmented algorithm. 
%%shou for each of them. 
The results are as follows:
\begin{itemize}
    \item [1.] Consider the sequence prediction without identity. For this arbitrary sequence case, we design an algorithm that is 
    %0416$1$-consistent and $3$-robust.
    $(1+\lambda)$-consistent and $(3+2/ \lambda)$-robust, where $\lambda \in (0,1]$ is a parameter describing the confidence level in the prediction.
    \item [2.] Consider a restricted model in which the sequence prediction has the same size as the set of actual requests. We propose a $\min \{3, 1 + (2\errortime + 4 \errorpos) / \costopt\}$-competitive algorithm, where $\errortime = max_{i \in [n]}|\hat{t}_i - t_i|$ is the maximum time difference between the predicted and actual requests and $\errorpos = \sum_{i}d(\hat{p}_i, p_i)$ is the accumulated distance between the predicted and actual positions. 
    \item [3.] Consider the prediction of the last arrival time. We design a $\min \{4, 2.5 + |\errorlast| / \costopt \}$-competitive polynomial-time algorithm, where $\errorlast = \hatt_n - t_n$ 
    %%shou is 
    denotes 
    the difference between the predicted and actual arrival time of the last request.
    %0403 Note that when the prediction is accurate, this competitive ratio is better than the best-known result of $2.65$ in~\cite{ascheuer2000online}. 
    %0403 It implies that even a small amount of information can really help improve the performance.
\end{itemize}
\smallskip
We also study the lower bounds for the OLTSP with predictions:
\smallskip
\begin{itemize}
    \item [1.] Consider the sequence prediction without identity. Any $1$-consistent algorithm has no robustness. We show there is a trade-off between consistency and robustness.
    \item [2.] Consider the sequence prediction with identity. Any $1$-consistent algorithm has a robustness that is at least 2.
    \item [3.] Consider the prediction of the last arrival time. We show that the consistency cannot be better than 2; 
    %%shou which means that 
    that is, 
    partial information is not enough for breaking the original lower bound of the OLTSP.
\end{itemize}
In addition, we extend our models to the 
%%shou more general 
online
dial-a-ride problem.

%\medskip
%%shou \noindent{\textbf{Outline.}}
% The paper is organized as follows. In Section~2 we introduce the formal definition of the problem and 
% %%shou
% three different types of predictions considered in this work. 
% %0406
% Then, in Section~3, we discuss two models with a sequence prediction and propose corresponding learning-augmented algorithms.
% %0406 when ignoring the computation time
% In Section~4 we consider the model with the predicted last arrival time 
% %%shou as prediction 
% and propose a polynomial-time algorithm. 
% %%shou for the OLTSP. 
% In Section~5 we extend the framework to the OLDARP. Finally, we 
% %%shou summarize and give 
% conclude with 
% some open problems for future studies in Section~6.

==> Online TSP with Predictions_v1r/sec_2_prelim.tex <==
\section{Preliminaries}\label{premlim}
In this section, we first give 
%%shou a 
the 
formal definition of the OLTSP, and 
%%shou then 
revisit the \PAH~algorithm, a key ingredient for 
%%shou proposing the models and 
designing our algorithms. Finally, we define error measurement for the 
%%shou different 
three
models. 



\subsection{The OLTSP}
Recall the metric OLTSP in which the input is a sequence of $n$ requests $\X = (x_1, \ldots, x_n)$
% , comprising $n$ requests 
in a metric space $M$. 
Each request $x_i \in \X$ can be represented 
%%shou as 
by $x_i = (t_i, p_i)$, where $t_i$ denotes the arrival time
% when the request is released and becomes known 
and $p_i$ denotes the position of the request. In addition, we assume the requests are in 
%%shou
non-decreasing order of arrival time; that is, $t_i \leq t_j$ for any $i < j$, and $t_n$ is the arrival time of the last request in $\X$. A server is required to start at the origin $o$ at time $0$, visit each request $x_i$ in $\X$ at position $p_i$ no earlier than its arrival time $t_i$, and at last come back to the origin $o$, which is also called home. Assuming the server moves with unit speed, the goal is to find a route $T_{\X}$ such that the completion time, denoted by $|T_{\X}|$, is minimized.

%%shou For 
\longdelete{
Regarding 
the previous results of the metric OLTSP without predictions, Ausiello et al.~\cite{ausiello2001algorithms} first studied this problem; they showed the lower bound of 2 and proposed an optimal algorithm, \PAH. Note that 
%%shou although the TSP is NP-hard, 
the \PAH~algorithm can yield a competitive ratio of 3 in polynomial time 
%%shou
using Christofides’ heuristic~\cite{worboys_1985}. 
%%
Ausiello et al.~\cite{ausiello2004algorithms} improved the polynomial-time result to $\frac{7+\sqrt{17}}{4}\approx 2.78$;  
%%shou by restricting the maximum distance of the server to the origin. 
on the other hand, 
Ascheuer et al.~\cite{ascheuer2000online} obtained the currently best 
%%shou result 
ratio of 
$\frac{7+\sqrt{13}}{4}\approx 2.65$ by leaving the server idle from time to time smartly.}
%0406 Note that if we do not care about the running time and assume the algorithm can access to the optimal route for a set of given requests, PAH is an optimal 2-competitive algorithm.

\medskip 
\noindent{\textbf{The \PAH~Algorithm~\cite{ausiello2001algorithms}.}}
Before introducing the proposed online algorithms with predictions, we first revisit 
%%shou an
the 
%%0403 optimal 
online algorithm, \textsc{Plan-At-Home (PAH)} for the OLTSP in a metric space, reported in~\cite{ausiello2001algorithms}, and see how we can attain 
%%shou
the robustness of our algorithms. The greedy \PAH~algorithm achieves a competitive ratio of $2$ when assuming the server can access an optimal solution 
%0403 of the offline TSP
to visit a set of released requests. Although the optimal route cannot be computed in polynomial time unless $P=NP$, 
%%shou
the \PAH~algorithm is $3$-competitive by using Christofides' heuristic~\cite{worboys_1985} to approximate the optimal route. 
%0420 In contrast to route $R$, which is subject to requests' arrival time, we denote $T$ as a route that visit a set of requests without time constraints and $|T|$ as the completion time of the route, whether the route is optimal or approximate. 
The details of the \PAH~algorithm can be referred to the Appendix~\ref{PAH:code}.

\begin{theorem}[\cite{ausiello2001algorithms}, Theorem 4.2]\label{thm:PAH2}
%%shou
The \PAH~algorithm is $2$-competitive for the OLTSP in a metric space.
\end{theorem}

\begin{theorem}[\cite{ausiello2001algorithms}, Theorem 5.3]\label{thm:PAH3}
%%shou
The \PAH~algorithm is a $3$-competitive polynomial-time algorithm for the OLTSP in a metric space when using Christofides' heuristic.
\end{theorem}

The overview of the \PAH~algorithm has the following two operations: (1) find a route only when the server is at the origin $o$, and (2) act differently in response to 
%%shou
the requests that are relatively close to the origin and those that are relatively far.
%0403 when the server is following a route
%%
%%shou
At moment $t$ during the execution of the algorithm, 
%%shou move here 
let $p(t)$ denote the position of the server 
%%shou at time $t$ 
%0403 operated by an algorithm 
and 
$U_t$ denote the set comprising 
%%shou the 
every 
unserved request that has been present 
%%shou at time $t$. 
so far. 
%%shou
Precisely, 
if the server is at the origin, i.e., $p(t)=o$, it starts to follow an optimal (or approximate) route $T_{U_t}$, which visits all released unserved requests in $U_t$
and returns to the origin $o$. 
%%shou
Otherwise,
when the server is on a route
%0420
$T_{U_{t'}}$, where $t' < t$ and $t'$ denotes the 
%%shou time 
moment when 
the route was designed, 
and a new request $x_i = (t_i, p_i)$ arrives, the server moves depending on the relationship between $d(p_i, o)$ and $d(p(t), o)$, where 
%0416 We use 
$d(a, b)$ denotes the shortest distance between points $a$ and $b$. If $d(p_i, o) > d(p(t), o)$, 
%%shou the
request $x_i$ is considered far from the origin, and the server terminates the route $T_{U_{t'}}$ and goes back to the origin $o$ directly. Otherwise, 
%%shou the 
request $x_i$ is considered close to $o$, and 
%%shou
thus the server ignores $x_i$ until it is back 
%%shou to the origin 
home 
and continues with 
the 
%%shou QQQ
current
route $T_{U_{t'}}$. 
%0420 For the simplicity, we use $T$ to replace $T_{U_{t'}}$ in the following section.

\longdelete{
\begin{algorithm}
\caption{\PAH
% Algorithm
}\label{alg:PAH}
    \begin{algorithmic}[1] %1: provides the line numbered at every line
    % \Procedure{\PAH}{The set of current released unserved requests $U_t$}
    %The actual input $\X$
    \Require The current time $t$ and the set of current released unserved requests $U_t$
    \State \textbf{If} the server is at the origin (i.e., $p(t) = o$) \textbf{then}
        \State \quad Start to follow an optimal (or approximate) route $T_{U_t}$ 
        %%shou which serves 
        passing through each 
        request in 
        \Statex \quad $U_t$.
    \State \textbf{ElseIf} the server is 
    currently moving along a route $T_{U_{t'}}$, for some $t' < t$ \textbf{then}
    % where $t' < t$
        \State \quad \textbf{If} a request $x_i = (t_i, p_i)$ arrives \textbf{then}
            \State \quad \quad \textbf{If} $d(p_i, o) > d(p(t), o)$ \textbf{then}
                \State \quad \quad \quad Go back to the origin $o$.
            \State \quad \quad \textbf{Else}
                \State \quad \quad \quad
                %%shou Continue 
                Move ahead
                on the current route $T_{U_{t'}}$.
            \State \quad \quad \textbf{EndIf}
        \State \quad \textbf{EndIf}
    \State \textbf{EndIf}
    % \EndProcedure
    \end{algorithmic}
\end{algorithm}
}

%%shou In the next sections where predictions are 
\begin{comment}
In order to 
incorporate predictions into the \PAH~algorithm, we use $L_{\PAH}(t, \X)$ to denote the completion time of the route $T$ that starts at the origin $o$ at time $t$ and serves the requests in $\X$ by implementing the \PAH~algorithm. Let $L_{Chr}(\X)$ be the completion time of the route $T$ found by Christofides' algorithm, which starts at the origin $o$ and serves the requests in set $\X$. 
%0403 
Let $L_{off}(\X)$ be the completion time of an offline optimal route that starts at the origin $o$ and serves the requests in $\X$, which arrive before the route is planned.
%0403
We have $L_{Chr}(\X) \leq 1.5 L_{off}(\X)$.
Note that since Christofides' algorithm and the offline solution does not consider the release time of the requests, the starting time of the route is irrelevant to the route's completion time.
\end{comment}

In addition, we can derive Corollary~\ref{cor:PAHwait} from the proof of \PAH~in~\cite{ausiello2001algorithms}.
\begin{corollary}\label{cor:PAHwait}
Assume an algorithm asks the server to wait at the origin $o$ for time $t$ before following the \PAH~algorithm where $t \leq t_n$. The algorithm is $2$-competitive if the server has access to the offline optimal route to serve a set of released requests. Also, it is $3$-competitive using Christofides' algorithm.
\end{corollary}

\begin{comment}
%0403 Due to the structure of the PAH algorithm, 
Considering a server operated by \PAH, if no request arrives after the server starts to follow a route $T$, the route will not be interrupted. Thus, we have Remark~\ref{rmk:equal}.

\begin{remark}\label{rmk:equal}
%0403 Let $t_n$ is the arrival time of the last request in sequence $\X$.
%0416 If $t \geq t_n$, then $L_{PAH}(t, \X) = L_{Chr}(\X)$.
If $t \geq t_n$, then $L_{\PAH}(t, \X) = L_{off}(\X)$.
\end{remark}
\end{comment}



\subsection{Prediction Models and Error Measure}
In this section, we present three different models of prediction.
%%shou we are studying. 
First, we consider 
%0406 a natural extension of 
predicting a sequence of requests $\Xpred = (\xhat_1, \ldots, \xhat_m)$, where $m$ denotes the number of predicted requests in the sequence. As the server is unaware of the size of $\X$ in the beginning, we assume that the learning model forecasts the number of requests before predicting the arrival time and positions of all requests. Formally, each request in the prediction is defined by $\xhat_i = (\hat t_i, \hat p_i)$, where $\hat t_i$ and $\hat p_i$ are its predicted arrival time and position. As we need to compare two request sequences with different sizes, $n$ and $m$, 
%%shou we assume that 
apparently 
a proper definition of prediction errors does not exist. Consequently, we only care about whether any error exists. That is, we simply distinguish whether $\Xpred = \X$ or not. In this model, we 
%%shou
can 
design an 
%0403 simple
algorithm that is consist and robust but not smooth. 

Next, we consider a restricted version 
%%shou that 
in which 
the number of requests $n$ is given, 
%%shou which 
implying that the prediction has the same size as the actual request sequence, i.e., $|\Xpred|=|\X|=n$. We 
%%shou
thus 
assume that there is a one-to-one 
%%shou relationship 
correspondence 
between the requests in the two sequences $\Xpred$ and $\X$. That is, each predicted request $\xhat_i$ is %%shou uniquely 
exactly 
paired 
%%shou to 
with 
the actual request $x_i$. Since the prediction gives us both the arrival time and position, we define errors with respect to the two parameters. We first define the time error, denoted by $\errortime$, as the maximum difference between the arrival time of a predicted request and its corresponding actual request.
$$\errortime \defeq max_{i \in [n]}|\hat{t}_i - t_i|$$
Then, we define the position error, denoted by $\errorpos$, as the sum of distances between the positions of the predicted and actual requests.
%%shou
$$\errorpos \defeq \sum^{n}_{i=1}d(\hat{p}_i, p_i)$$
%%shou Extending from the algorithm designed for the previous model, 
In this restricted model, 
we extend the above algorithm to 
%%shou propose another algorithm to 
a new one which can 
improve the result and satisfy the smoothness requirement. 
 
 
Last, we consider the prediction 
%%shou which is 
of 
the arrival time of the last request, 
%%shou and denote this value 
denoted 
by $\hat t_{last}$. We define the error of the prediction, denoted by $\errorlast$, 
%%shou as 
to be 
the difference between the predicted and the actual arrival time of the last request: 
$$\errorlast \defeq \hatt_n - t_n.$$
%%
The motivation of 
%%shou choosing this 
making such a 
prediction is that the arrival time of the last request provides a guess of the lower bound for the optimal route. 
%%shou In the following sections, 
Later 
we show how to combine this prediction with the \PAH~algorithm and design a learning-augmented algorithm
with consistency, robustness and smoothness. Furthermore, we also show the limit of this prediction, 
%%shou QQQ
i.e., lower bound results.


Note that $\Xpred$ 
%%shou provides 
reveals 
much more information compared to $\hatt_n$ so that 
%%shou we can expect 
the first two prediction models 
%%shou can 
would be expected to 
help achieve better 
%%shou results 
performance 
than the last model, 
%%shou when 
assuming 
the prediction is perfect. 
%0403 scenario
However, 
when the prediction is not 
%%shou so perfect
good, 
we 
%%shou need to 
must carefully 
control both $\errortime$ and $\errorpos$ to avoid paying too much 
%%shou
extra cost.

Here we 
%%shou mentioned 
remark 
that very recently Azar et.al.~\cite{azar2022online} proposed a framework for designing learning-augmented online 
%%shou graph 
algorithms for some graph problems such as Steiner tree/forest, facility location, etc. 
% receives a set of locations as the prediction while the number of requests is unknown, and 
They also 
%%shou propose 
presented 
a novel definition of prediction errors. However, 
%%shou
in contrast, 
%%shou in the OLTSP, we have 
online routing has to
%%shou to consider the 
carefully cope with the predictions of 
arrival time of future requests. Therefore, the notion 
%%shou proposed 
reported 
in~\cite{azar2022online} may not be 
%%shou the best choice for 
directly applied to 
this study.


==> Online TSP with Predictions_v1r/sec_3_a_sequence_of_requests.tex <==
\section{Predict a Sequence of Requests}\label{pred:seq}

%%shou consider the models with sequence prediction 
Given a predicted sequence of requests
$\Xpred$, 
we first discuss the intuition behind the 
%%shou
two models: 
\emph{prediction without identity} and \emph{prediction with identity}. 
%%shou Another question is how the learning models predict. 
%%shou We consider two types of sequence prediction: 
%%shou
From the perspective of machine learning, 
the former model forecasts by viewing the sequence as a whole, while the latter one makes predictions based on the features of each request individually. Note that both models acquire the entire sequence prediction $\Xpred$ in the beginning. 
Next,
we present two algorithms: \algNI~and \algI, respectively, where  
%%shou , which  
the former one has
consistency and robustness, and 
%%shou Finally, we show that algorithm~\algI~
the latter one can even additionally
gain smoothness 
%%shou in addition to those two properties 
by knowing the number of requests.
%%


%%shou
We remark that, analogous to the discussion in~\cite{ausiello2001algorithms}, 
one can 
disregard the computational complexity of online algorithms and 
%%shou focus on the case where 
assume that 
the server has access to the offline optimal route for a sequence of 
%%shou
released requests. 
%%shou with release time. Note that 
%%
%0416 by contrast, Ausiello et al.~\cite{ausiello2001algorithms} assume 
%%shou
This is 
%%shou in contrast 
similar 
to the assumption in~\cite{ausiello2001algorithms} that 
the server is given the optimal solution to visit requests without time constraints. 
%0412-HT As Theorem~\ref{thm:>2} shows, an algorithm with merely prediction of the last arrival time $\hat t_{last}$ cannot be better than $2$-competitive. Therefore, we need prediction with more information in this setting.
%0403 of a vehicle routing problem. Note that whereas the server of an online algorithm has access to the optimal solution of a traveling salesman problem in~\cite{ausiello2001algorithms}, we assume the server of a learning-augmented algorithm has access to that of a vehicle routing problem.
%0403


%0403 The former one makes predictions based on the characteristics of each request individually, given the number of requests in the sequence; the latter one forecasts based on the features of a sequence as a whole.



\begin{comment}
\begin{algorithm}
\caption{Adjusted-PAH Algorithm}\label{alg:adjustedPAH}
    \begin{algorithmic}[1] %1: provides the line numbered at every line
    %\Procedure{Adjusted PAH}{The end time $t_{end}$, the set of current unserved requests $U$}
    %The actual input $\X$
    \Require The end time $t_{end}$, and the set of current unserved requests $U$
    \State \textbf{If} the server is at the origin $o$ (i.e., $p(t) = o$.) \textbf{then}
        \State \quad Compute an approximate route $T$ to serve all the unserved requests in $U$ and return
        \Statex \hspace{22pt} to the origin $o$;
        \State \quad \textbf{If} $t < t_{end}$ and $t + |T| > t_{end}$ \textbf{then}
            \State \quad \quad Find a time $t_{back}$ such that $t_{back} + d(p(t_{back}), o) = t_{end}$;
            \State \quad \quad Redesign a route $T''_{U_t}$ by asking the the server to go back to the origin $o$ at time
            \Statex \hspace{33pt} $t_{back}$ along the shortest path;
            \State \quad \quad Start to follow the route $T''_{U_t}$.
        \State \quad \textbf{Else}
            \State \quad \quad Start to follow the route $T$.
        %0403
        \State \quad \textbf{EndIf}
    \State \textbf{ElseIf} the server is currently following a route $T'$ \textbf{then}
        \State \quad \textbf{If} a new request $x_i = (t_i, p_i)$ arrives \textbf{then}
            \State \quad \quad Interrupt the route $T'$ and go back to the origin $o$ along the shortest path.
        \State \quad \textbf{Else}
            \State \quad \quad Continue on the current route $T'$.
        %0403
        \State \quad \textbf{EndIf}
    %0403
    \State \textbf{EndIf}
    %\EndProcedure
    \end{algorithmic}
\end{algorithm}
\end{comment}


%0406 \noindent{\textbf{The Adjusted-PAH procedure.}}
%0406 TODO: describe the procedure

\subsection{Sequence Prediction without Identity}\label{sec:3-1}
In this model, the server 
%%shou receives 
makes 
a prediction $\Xpred$ 
%%shou containing 
comprising 
$m$ predicted requests.
%0412HT, which is the predicted number of requests. 
We present the~\algNI~algorithm, which is $(1.5+\lambda)$-consistent and $(3+2/\lambda)$-robust for $\lambda \in (0, 1]$. 
%0406 The idea is that the server trusts the prediction $\Xpred$ in the beginning but switches back to the PAH algorithm once an error is detected. 
%0406 The idea is that the server find a predicted optimal route $\hat T$ for the prediction $\Xpred$ but do not follow the route at time $0$. Instead, it postpone the route for a while and follow the PAH algorithm during this period. To obtain robustness, the server follows the route $\hat T$ only when it finds a proper lower bound for the optimal completion time $\costopt$. 
%%shou
A na\"{\i}ve idea is that the server finds an 
%%shou predicted 
optimal route $\hat T$ for the prediction $\Xpred$ at time $0$ and 
just 
follows the route $\hat T$ 
%%shou after it finds a proper lower bound for the optimal completion time $\costopt$.
%
%%shou If we follow the predicted optimal route $\hat T$ 
directly.
%0416 which 
It is clearly a 1-consistent algorithm, which, however, 
%%shou we show that it 
may 
%%shou lead to 
result in 
an arbitrarily bad robustness.


\begin{restatable}{rThm}{thmlbwo}\label{thm:lb1}
Given a sequence of predicted requests without identity, 
%%shou as the prediction, 
any 1-consistent algorithm has robustness 
%%shou
of at least $1/\delta$
%0419 where
for any $\delta \in (0,1)$.
%,  with sequence prediction without identity. \textcolor{red}{Need more assumption for the identity? Otherwise, it contradicts to the results of Theorem 12}
\end{restatable}
% \begin{proof}
% Consider the 
% %%shou
% OLTSP on the real line, a special metric space. 
% Let the prediction be $\Xpred = \{x_1 = (\delta, \delta), x_2 = (1, 1)\}$, where $\delta \in (0, 1)$.
% First, 
% %%shou we assume that 
% suppose 
% the actual input is $\X = \Xpred$. In this case, the
% offline
% optimal solution is to start moving at time $0$, visit $x_1$ at time $\delta$ and $x_2$ at time $1$, and return to the origin at time $2$. To obtain the consistency of $1$, the server must follow the exact same route as the optimal one.
% On the other hand, 
% %%shou we assume another 
% if the 
% actual input is $\X' = \{x'_1 = (\delta, \delta)\}$, 
% %%shou
% i.e. only one request. 
% %%shou Note that 
% Since the number of requests is unknown, the algorithm recognizes the error at time $1$ and cannot 
% %%shou return to the origin $o$ before 
% go back home until 
% time $2$. However, the offline optimal 
% %%shou route 
% solution 
% finishes at time $2 \delta$. Thus, the competitive ratio is $\costalg / \costopt \geq 2 / (2 \delta) = 1 / \delta$.
% \end{proof}


The brief idea of the~\algNI~algorithm is that the server finds an 
%%shou predicted 
optimal route $\hat T$ for the prediction $\Xpred$ at time $0$ and follows the route 
based on a modified framework of \PAH, which can guarantee a lower bound for 
%%shou $\hat T$ after it finds a proper lower bound for the optimal completion time 
$\costopt$.
%%
%%shou Specifically, 
Precisely,
a server operated by \algNI~is given a route $\hat T$ which serves 
%%shou
the requests in the prediction $\Xpred$ 
%%shou and the 
with 
the confidence level to the prediction, denoted by $\lambda$, in the beginning. To obtain 
%%shou
certain 
robustness, 
we set a condition to see whether the current moment $t$ is 
%%shou before or after 
earlier than 
$\lambda |\hat T|$ or not. 
%%shou When 
If 
$t < \lambda |\hat T|$, we 
follow
the \PAH~algorithm, unless the route $T_{U_t}$ is too long (i.e., $t + |T_{U_t}| >  \lambda |\hat T|$), where 
$T_{U_t}$ denotes an optimal route that starts serving the set of released unserved requests $U_t$ at time $t$; that is, we adjust the route $T_{U_t}$ by asking the server to 
%%shou go back to the origin $o$ at time $t_{back}$
return home and arrive at the origin $o$ exactly at time $\lambda |\hat T|$.
%%shou otherwise, the server follows the \PAH~algorithm. 
%%
By 
%%shou doing so, 
adding such a gadget, 
we can ensure 
%%shou
good robustness. 
%%shou that the server can be at the origin $o$ at time $\lambda |\hat T|$. Then, after 
Otherwise, 
if $ t \ge \lambda |\hat T|$, 
the server 
%%shou starts 
gets 
to follow the predicted route $\hat T$ 
%%shou when 
once 
there are unserved requests (i.e., $U_t \neq \emptyset$). 
%%shou
Finally, we use the \PAH~algorithm to serve the remaining requests in $\X \setminus \Xpred$ . 
Note that we tend to set the parameter $\lambda$ to a small value if we believe the quality of the prediction is good. 


\begin{comment}
If the server cannot visit all requests in $\X$ with the route $\hat T$, which implies that some request in $\X$ is not in $\Xpred$, we use the \PAH~algorithm to serve the remaining ones. 

the server does not follow the route $\hat T$ at time $0$. It starts following the \PAH~algorithm at time $0$ and asks the server to be back to the origin $o$ at time $\lambda |\hat T|$. If the server cannot visit all requests arrived before $\lambda |\hat T|$, it starts to follow the predicted route $\hat T$. Otherwise, it waits at the origin $o$ until the next request arrives before following $\hat T$. After that, it switches back the \PAH~algorithm and completes the task.
\end{comment}

%0416 We let $U_t$ denote the unserved request that has been present at the time $t$. 
%
%%shou By Theorem~\ref{thm:LASwo}, 
In particular, 
next, we show that~\algNI~can still be robust even when the prediction error is not properly defined.
First, we prove it is feasible to add the gadget. 

%start to follow a route $\hat T$ designed for requests in $\Xpred$, 

%0406 NOTE: the existence of $t_{back}$ should be moved to here.


\begin{restatable}{rLem}{lemtback}\label{lem:tback}
%0416 Given that the server follows Algorithm~\ref{alg:replan}, let $T$ be an approximate route that start serving a set of released requests at time $t$. If the time $t$ satisfies that $t < \hat t_{last}$ and $t + |T| > \hat t_{last}$, there exist a time $t_{back} \in (t, t + |T|)$ such that $t_{back} + d(p(t_{back}), o) = \hat t_{last}$.
Given that the server follows the~\algNI~algorithm, 
%%shou if 
when time $t$ satisfies the condition: $t < \lambda |\hat T|$ and $t + |T_{U_t}| > \lambda |\hat T|$, there exist a %%shou time
moment $t_{back}$, $t < t_{back} < t + |T_{U_t}|$, such that $t_{back} + d(p(t_{back}), o) = \lambda |\hat T|$.
\end{restatable}
% \begin{proof}
% Define the function $f: [t, t + |T_{U_t}|] \rightarrow [t, t + |T_{U_t}|]$ 
% %%shou as the
% %0403 completion time of the route 
% to be 
% %%shou time 
% the moment 
% when the server arrives at the origin again; 
% %%shou
% that is, 
% the server stops following route $T_{U_t}$ and goes back to the origin 
% %%shou $o$ 
% at a particular moment $t_{back}$, i.e., $f(t_{back}) = t_{back} + d(p(t_{back}), o)$. 
% Then, 
% %%shou
% we let the function $g(x) \defeq f(x)-\lambda |\hat T|$, 
% %%shou
% and it has two properties: $g(t) = t - \lambda |\hat T| < 0$ and $g(t + |T_{U_t}|)= t + |T_{U_t}| -\lambda |\hat T| > 0$. Since $g$ is continuous, there must be at least one point $t_{back}\in (t, t + |T_{U_t}|)$ such that $g(t_{back})= 0$ and 
% %%shou
% thus $t_{back} + d(p(t_{back}), o) = \lambda |\hat T|$. Without loss of generality, 
% we choose the last one 
% %%shou QQQ
% satisfying $g(t_{back})= 0$.
% \end{proof}

\begin{algorithm}
    % \caption{An Algorithm with Sequence Prediction without Identity}
    \caption{\textsc{Learning-Augmented Routing Without Identity (LAR-NID)}}
    \label{alg:LASwo}
    \begin{algorithmic}[1] %1: provides the line numbered at every line
    \Require The current time $t$, a sequence prediction $\Xpred$, the confidence level $\lambda \in (0, 1]$, and the set of current released unserved requests $U_t$.
    \State 
    %%shou Initially, 
    First, 
    compute an optimal route $\hat T$ to serve 
    %%shou
    the requests in $\Xpred$ and return to the origin $o$;
    \State \textbf{While} $t < \lambda |\hat T|$ \textbf{do}
        \State \quad \textbf{If} the server is at the origin $o$ (i.e., $p(t) = o$.) \textbf{then}
            \State \quad \quad Compute an optimal route $T_{U_t}$ to serve all the unserved requests in $U_t$ and return
            \Statex \quad \quad to the origin $o$;
            \State \quad \quad \textbf{If} $t + |T_{U_t}| >  \lambda |\hat T|$ \textbf{then}
            \Comment{Add a gadget}
                \State \quad \quad \quad Find
                %%shou a time 
                the moment 
                $t_{back}$ such that $t_{back} + d(p(t_{back}), o) =  \lambda |\hat T|$;
                \State \quad \quad \quad Redesign a route $T'_{U_t}$ by asking the the server to go back to the origin $o$ at time
                \Statex \quad \quad \quad $t_{back}$ along the shortest path;
                \State \quad \quad \quad Start to follow the route $T'_{U_t}$.
            \State \quad \quad \textbf{Else}
                \State \quad \quad \quad Start to follow the route $T_{U_t}$.
            %0403
            \State \quad \quad \textbf{EndIf}
        \State \quad \textbf{ElseIf} the server is currently 
        %%shou following 
        moving along 
        a route $T_{U_{t'}}$, for some $t'< t$ \textbf{then}
            \State \quad \quad \textbf{If} a new request $x_i = (t_i, p_i)$ arrives \textbf{then} 
            %%shou             
            \Comment{Similar to PAH}               
            \State \quad \quad \quad \textbf{If} $d(p_i, o) > d(p(t), o)$ \textbf{then}
                    %0406 \State \quad \quad \quad \quad Interrupt the route $T'$ and go back to the origin $o$ along the shortest path.
                    \State \quad \quad \quad \quad Go back to the origin $o$.
                \State \quad \quad \quad \textbf{Else}
                    \State \quad \quad \quad \quad 
                    %%shou Continue 
                    Move ahead 
                    on the current route $T_{U_{t'}}$.
                \State \quad \quad \quad \textbf{EndIf}
            %0403
            \State \quad \quad \textbf{EndIf}
        %0403
        \State \quad \textbf{EndIf}
    \State \textbf{EndWhile}
    
    \State \textbf{While} $t \geq \lambda |\hat T|$ \textbf{then}
        %0406 \State \quad Wait until $t'$ such that $t'$ is the first moment when $U \neq \emptyset$.
        %0406 \State \quad Wait until $t'$ such that $t' = \min_{t} \{t \geq \lambda |\hat T| : U_t \neq \emptyset \}$;
        \State \quad Wait until $U_t \neq \emptyset$;
        \State \quad Follow the route $\hat T$ until the server is back to the origin $o$;
        %0406 \State \quad Follow PAH algorithm.
        \State \quad Follow \PAH~($t,U_t$).
        \Comment{Serve the remaining requests}
    \State \textbf{EndWhile}
    \end{algorithmic}
\end{algorithm}


%%shou

\begin{restatable}{rLem}{lemconsistency}\label{lem:consistency}
The~\algNI~algorithm is $(1.5 + \lambda)$-consistent, where $\lambda \in (0,1]$.
\end{restatable}
% \begin{proof}
% %0406 is an optimal route. 
% The server 
% %%shou starts 
% gets 
% to follow the 
% %%shou adjusted version 
% modified framework 
% of the \PAH~algorithm at time $0$ and returns to the origin at 
% exactly 
% time $\lambda |\hat T|$. Then, at time $\lambda |\hat T|$, the server 
% %%shou either 
% follows the predicted route $\hat T$
% %%shou immediately 
% if  $U_{\lambda |\hat T|} \neq \emptyset$; 
% %%shou or
% otherwise, it waits until the next request arrives. 
% %%
% Assume the prediction is perfect, i.e., $\Xpred = \X$ and $|\hat T| = \costopt$.
% Since $\hat T$ is an optimal route, the server completes after following $\hat T$.
% %%shou Then, 
% We consider the following two cases:

% \begin{itemize}
%     \item {1. $U_{\lambda |\hat T|} \neq \emptyset$.} In this case, the server gets to follow route $\hat T$ at time $\lambda |\hat T|$, and the completion time of the algorithm is $\costalg = \lambda |\hat T| + |\hat T| \leq (1 + \lambda) \costopt$. 
%     \item {2. $U_{\lambda |\hat T|} = \emptyset$.} In this case, after time $\lambda |\hat T|$, the server waits for the next request to 
%     %%shou come. 
%     move. 
%     Let $x_j = (t_j, p_j)$ denote this request, which implies 
%     %%shou QQQ > instead of \geq
%     $t_j = \min_t \{t > \lambda |\hat T| : U_t \neq \emptyset \}$. The completion time of the algorithm is $\costalg = \lambda |\hat T| + (t_j - \lambda |\hat T|) + |\hat T|$. Note that $t_j - \lambda |\hat T|$ is the time length
%     %0416 interval 
%     that the server waits at the origin. 
%     %%shou $o$. Then, 
%     We split the duration $t_j - \lambda |\hat T|$ into two time intervals according to the operations of the offline optimal server, 
%     %%shou QQQ
%     i.e., OPT: 
%     %0416perform
%     $t_{move}$ and $t_{idle}$. 
%     %%shou
%     The former denotes how much time 
%     %%shou an optimal server 
%     the OPT
%     is moving, and 
%     %%shou $t_{idle}$ 
%     the latter
%     denotes the time length 
%     %%shou of time 
%     the 
%     %%shou optimal server 
%     OPT
%     %%shou QQQ   has nothing to do and can only wait until the next request to come, where 
%     just waits at the origin. 
%     That is, 
%     $t_{move} + t_{idle} = t_j - \lambda |\hat T|$. Note that 
%     %%shou the server operated by the algorithm 
%     \algNI~is 
%     not visiting any request during $t_{idle}$, 
%     %%shou
%     either. Because 
%     the case $t_{idle} \neq 0$ favors the algorithm, 
%     we simply 
%     %%shou assume 
%     consider
%     the worst case $t_{idle} = 0$ and thus $t_{move} = t_j - \lambda |\hat T|$. Intuitively, the 
%     %%shou optimal server 
%     OPT
%     gains the advantage by moving toward the next request 
%     %%shou it plans to serve 
%     during $t_{move}$. 
%     %%shou In addition, we know 
%     Moreover, 
%     the time/distance 
%     %%shou it 
%     the OPT
%     saves by moving earlier 
%     %%shou than the online server cannot be longer than 
%     is at most 
%     $\frac{1}{2} \costopt$ 
%     %%shou ; otherwise, by applying 
%     due to 
%     the triangle inequality. 
%     %%shou the total length of the offline optimal route will be larger than $\costopt$ which leads to a contradiction. 
%     %%
%     Since the server moves at unit speed, we have $t_{move} \leq \frac{1}{2} \costopt$. To sum up, the completion time is $\costalg \leq \lambda |\hat T| + t_{move} + |\hat T| \leq (1.5 + \lambda) \costopt$.
% \end{itemize}
% \end{proof}

\begin{restatable}{rLem}{lemrobustness}\label{lem:robustness}
The~\algNI~algorithm is $(3 + 2 / \lambda)$-robust, where $\lambda \in (0,1]$.
\end{restatable}
% \begin{proof}
% % We consider $\Xpred \neq \X$ and 
% Note that $t_i \leq Z^{OPT}$ for any $i$ and $|T_{U_{t}}| \leq Z^{OPT}$ for any $t$.
% To show the robustness, we consider the following cases: 

% \begin{itemize}
%     %%shou
%     \item {1. Assume the server finishes before $\lambda |\hat T|$.} In this case, the server acts exactly like the \PAH~algorithm and does not follow route $\hat T$. 
%     % would do. 
%     Thus, by Theorem~\ref{thm:PAH2}, the server obtains the bound $\costalg \leq 2 \costopt$.
%     \item {2. The server cannot finish before $\lambda |\hat T|$.} In this case, there are some unserved requests at time $\lambda |\hat T|$ or some request 
%     %%shou
%     arriving after time $\lambda |\hat T|$. In both cases, the algorithm first follows $|\hat T|$ and then switches to the \PAH~algorithm if there 
%     %%shou
%     remain some unserved requests. Also, since the algorithm cannot serve all of the requests before time $\lambda |\hat T|$, it implies that $\costopt \ge \lambda |\hat T|/2$; otherwise, 
%     it contradicts Theorem~\ref{thm:PAH2}.
%     %0420 by Theorem~\ref{thm:PAH2}, the server can finish all of the requests by time $\lambda |\hat T|$.
%     To analyze the performance of 
%     %%shou our algorithm 
%     \algNI~in this case, we 
%     %%shou break 
%     divide
%     the case into the following four subcases: 
%     % After following $|\hat T|$, we cannot guarantee all requests have been served so the server switches to the PAH algorithm.
%         \begin{itemize}
%             \item{2-1. $U_{\lambda |\hat T|} \neq \emptyset$ and $t_n > (1 + \lambda)|\hat T|$.} 
%             % In this case, 
%             Since the~\algNI~algorithm follows \PAH~after time $(1 + \lambda)|\hat T|$, we have $\costalg \leq 2 \costopt$ by Corollary~\ref{cor:PAHwait}.
%             \item{2-2. $U_{\lambda |\hat T|} \neq \emptyset$ and $t_n \leq (1 + \lambda)|\hat T|$.} 
%             % In this case, 
%             By using $\lambda |\hat T| / 2 \leq Z^{OPT}$,
%             the completion time of the algorithm can be 
%             %%shou computed 
%             derived 
%             as follows: 
%             \begin{align*}
%                 \costalg & \leq \lambda |\hat T| + |\hat T| + |T_{U_{(1+\lambda)|\hat T|}}|
%                 \\& \leq 2 \costopt + (2 / \lambda) \costopt + \costopt
%                 \\& \leq (3 + 2 / \lambda) \costopt
%             \end{align*}
%             \item{2-3. $U_{\lambda |\hat T|} = \emptyset$  and $t_n > t_j + |\hat T|$.} This case is similar to the case 2-1. 
%             % In this case, 
%             The~\algNI~algorithm follows \PAH~after time $t_j + |\hat T|$. Thus, we have $\costalg \leq 2 \costopt$ by Corollary~\ref{cor:PAHwait}.
%             \item{2-4. $U_{\lambda |\hat T|} = \emptyset$  and $t_n \leq t_j + |\hat T|$.} 
%             % In this case, 
%             Some request arrives when the server is on the route $\hat T$, which implies that $\lambda |\hat T| < t_n \leq Z^{OPT}$. Also, the server starts its 
%             %%shou final 
%             last route at time $t_j + |\hat T|$, when it is back 
%             %%shou to the origin $o$.
%             home. 
%             The completion time of~\algNI~can be 
%             %%shou computed 
%             obtained 
%             as follows: 
%             \begin{align*}
%                 \costalg & \leq t_j + |\hat T| + |T_{U_{t_j + |\hat T|}}|
%                 \\& \leq \costopt + (1 / \lambda) \costopt + \costopt
%                 \\& \leq (2 + 1 / \lambda) \costopt
%             \end{align*}
%         \end{itemize}
% \end{itemize}
% %%shou
% The proof is complete. 
% \end{proof}

\begin{restatable}{rThm}{thmLASwo}\label{thm:LASwo}
The~\algNI~algorithm is $(1.5 + \lambda)$-consistent and $(3 + 2 / \lambda)$-robust
%%shou QQQ and 
but 
not smooth, where $\lambda \in (0,1]$ is the confidence level.
\end{restatable}
%%shou
\begin{comment}
\begin{proof}
%We discuss the consistency and robustness separately. 
By combining Lemma~\ref{lem:consistency} and Lemma~\ref{lem:robustness}, we thus derive the result. 
\end{proof}
\end{comment}


\subsection{Sequence Prediction with Identity}\label{sec:3-2}
In contrast to the previous model, we consider having access to the number
%%shou quantity 
of requests, i.e., $n$. 
%%shou and the 
%%shou
Given a 
sequence prediction, $\Xpred$ with the size of $n$, 
we first show 
%%shou that 
the limitation of this stronger prediction. 

\begin{restatable}{rThm}{thmlbw}\label{thm:lb2}
Given a sequence of predicted requests with identity, 
%%shou as the prediction, 
any $1$-consistent algorithm has robustness at least $2$. 
% ???
\end{restatable}


We first consider a 
%%shou na\"{\i}ve 
naive
algorithm, \algT, and
% (described in  Algorithm~\ref{alg:naive}) 
show that it is consistent and smooth but not robust where the details can be founded in the Appendix~\ref{naivealgo}. 
However, we observe that the arrival time of the last request $t_n$ gives a lower bound of the optimal solution, $\costopt$.
As a result, we modify the 
% na\"{\i}ve 
\algT~algorithm and propose the~\algI~algorithm, which is $1$-consistent, $3$-robust and $(2 \errortime + 4 \errorpos)$-smooth.


\begin{algorithm}
    % \caption{A Na\"{\i}ve Algorithm}
    \caption{\textsc{Learning-Augmented Routing Trust (LAR-Trust)}}\label{alg:naive}
    \begin{algorithmic}[1] %1: provides the line numbered at every line
    \Require The current time $t$, the number of requests $n$, a sequence prediction $\Xpred$, and the set of current released unserved requests $U_t$.
    \State 
    %Initially, First, 
    Compute an optimal route $\hat T = (\hat x_{(1)}, \ldots, \hat x_{(n)})$ to serve the requests in $\Xpred$ and return to the origin $o$, where $\hat x_{(i)} = (\hat t_{(i)}, \hat p_{(i)})$ 
    %%shou is 
    denotes
    the $i^{th}$ predicted request 
    %%shou to serve 
    in $\hat T$;
    \State Start to follow the route $\hat T$;
    \State \textbf{For} any $i =1, \ldots, n$ \textbf{do}
    
        \State \quad \textbf{If} $t = t_{(i)}$ 
        %0420 for any $i$ 
        \textbf{then}
            \State \quad \quad Update the route $\hat T$ by adding the request $x_{(i)}$ after the 
            %%shou
            predicted request $\hat x_{(i)}$;
            %0403 and $\hat x_{(i)}$
        \State \quad \textbf{EndIf}
        \State \quad \textbf{If} $p(t) = \hat p_{(i)}$ and $t < t_{(i)}$ \textbf{then}
            \State \quad \quad Wait at position $\hat p_{(i)}$ until time $t_{(i)}$.
            \Comment{Wait until the request arrives}
        \State \quad \textbf{EndIf}
    
    \State \textbf{EndFor}
    \end{algorithmic}
\end{algorithm}

\begin{restatable}{rThm}{thmnaive}\label{thm:naive}
% \begin{theorem}\label{thm:naive}
%0406 For the na\"{\i}ve algorithm, we have $\costalg \leq \costopt + 2 \errortime + 4 \errorpos$.
The competitive ratio of the~\algT~algorithm
% \ref{alg:naive} 
is $1 + 2 \errortime + 4 \errorpos$.
%0406, where $\errortime$ is the time error and $\errorpos$ is the position error. 
Thus, the algorithm is $1$-consistent and $(2 \errortime + 4 \errorpos)$-smooth but not robust.
\end{restatable}

% % \begin{comment}
% \begin{theorem}
% Any $1$-consistent algorithm with sequence prediction with identity has robustness at least $2$. 
% % ???
% \end{theorem}
% % \end{comment}





The intuition of the~\algI~algorithm is to keep the impact of errors under control. Specifically, the server finds an optimal route $\hat T$ to serve 
%%shou
the requests in $\Xpred$ in the beginning. Before time $t_n$, the server follows the route $\hat T$ and adjusts it when necessary. To explain how we make adjustments, we describe the route $\hat T$ as a sequence of requests that are in order of priority. That is, $\hat T \defeq (\xhat_{(1)}, \ldots, \xhat_{(n)})$ where $\xhat_{(i)} = (\hat t_{(i)}, \hat p_{(i)})$ 
%%shou is 
denotes 
the $i^{th}$ request 
%%shou
to be served in $\hat T$. If a request $x_i$ arrives, the server modifies the route $\hat T$ by inserting the request $x_{(i)}$ into the sequence $\hat T$ 
%0416 between requests $\xhat_{(i)}$ and $\xhat_{(i+1)}$. 
after the request $\xhat_{(i)}$.
By updating the route, the server can visit each request $x_i$ with the adjusted version of the route $\hat T$. When the last request $x_n$ arrives (i.e., $t = t_n$), we compute the length of our two possible routes: (1) the remaining distance of $\hat T$ after updates,
denoted 
%%shou as 
by
$r_1$, and (2) the distance to go back to the origin and follow the final route $T_{U_{t_n}}$ to visit the requests in $U_{t_n}$,
denoted 
%%shou as 
by 
$r_2$. Then, the server chooses the shorter one to visit the remaining requests in $\X$.
For (1), we can rewrite it as the na\"{\i}ve algorithm by updating the route sequentially, where the details can be
% referred to Algorithm~\ref{alg:naive} 
founded in the Appendix~\ref{naivealgo}.
We first show that the cost of the~\algT~algorithm
%0420~\ref{alg:naive} 
is associated with the error 
%%shou that we 
defined in Section~\ref{premlim}. Note that the server does not change the order to serve the requests in $\X$ unless the server gives up the route $\hat T$ at time $t_n$.

% \end{theorem}


\begin{algorithm}[!ht]
    % \caption{An Algorithm with Sequence Prediction with Identity}
    \caption{\textsc{Learning-Augmented Routing With Identity (LAR-ID)}}\label{alg:LASw}
    \begin{algorithmic}[1] %1: provides the line numbered at every line
    \Require The current time $t$, the number of requests $n$, a sequence prediction $\Xpred$, and the set of current released unserved requests $U_t$.
    \State $F = 0$;
    \Comment{Initialize $F=0$ to indicate that we trust the prediction} %% at first}
    \State 
    %0420 Initially, 
    First, compute an optimal route $\hat T = (\xhat_{(1)}, \ldots, \xhat_{(n)})$ to serve the requests in $\Xpred$ and return to the origin $o$, where $\xhat_{(i)} = (\hat t_{(i)}, \hat p_{(i)})$ is the $i^{th}$ request to serve in $\hat T$;
    \State Start to follow the route $\hat T$;
    
    \State \textbf{While} $F = 0$ \textbf{do}
    \Comment{Trust the prediction}
        \State \quad \textbf{If} $t = t_{(i)}$ 
        % for any $i$ 
        \textbf{then}
            % \State \quad \quad Update the route $\hat T$ by adding request $x_{(i)}$ between requests $\xhat_{(i)}$ and $\xhat_{(i+1)}$;
            \State \quad \quad $\hat T = (\xhat_{(1)}, \ldots, \xhat_{(i)}, x_{(i)}, \xhat_{(i+1)},  \ldots, \xhat_{(n)})$, for $i = 1, \ldots, n$;
            %0403 and $\hat x_{(i)}$
            \Comment{Update the route}
            \State \quad \quad \textbf{If} $t = t_n$ \textbf{then}
            \Comment{Find the shorter route}
                \State \quad \quad \quad $r_1 \leftarrow$ the remaining distance of following $\hat T$;
                \State \quad \quad \quad Compute a route $T_{U_{t_n}}$ to start and finish at the origin $o$ and serve the requests in 
                \Statex \quad \quad \quad $U_{t_n}$;
                \State \quad \quad \quad $r_2 \leftarrow d(p(t), o) + |T_{U_{t_n}}|$;
                \State \quad \quad \quad \textbf{If} $r_1 > r_2$ \textbf{then}
                    \State \quad \quad \quad \quad Go back to the origin $o$;
                    \Comment{Give up the predicted route}
                    \State \quad \quad \quad \quad $F = 1$.
                %0403
                \State \quad \quad \quad \textbf{Else}
                    \State \quad \quad \quad \quad 
                    %0420Continue 
                    Move ahead on the current route $\hat T$.
                \State \quad \quad \quad \textbf{EndIf}
            %0403
            \State \quad \quad \textbf{Else}
                \State \quad \quad \quad
                %0420Continue 
                Move ahead on the current route $\hat T$.
            \State \quad \quad \textbf{EndIf}
        \State \quad \textbf{EndIf}
        
        \State \quad \textbf{If} $p(t) = \hat p_{(i)}$ and $t < t_{(i)}$ \textbf{then}
            \State \quad \quad Wait at position $\hat p_{(i)}$ until time $t_{(i)}$.
            \Comment{Wait until the request arrives}
        \State \quad \textbf{EndIf}
    \State \textbf{EndWhile}
    \State \textbf{While} $F = 1$ \textbf{do}
    \Comment{Do not trust the prediction}
        \State \quad Start to follow the route $T_{U_{t_n}}$ to serve the requests in $U_{t_n}$.
    \State \textbf{EndWhile}
    \end{algorithmic}
\end{algorithm}

\begin{restatable}{rThm}{thmLASw}\label{thm:LASw}
The competitive ratio of the~\algI~algorithm is $\min \{3, 1 + (2 \errortime + 4 \errorpos) / \costopt\}$. Thus, the algorithm is $1$-consistent, $3$-robust and $(2 \errortime + 4 \errorpos)$-smooth.
\end{restatable}
% \begin{proof}
% Initially, the server follows an optimal route $\hat T$ for the requests in $\Xpred$,
% %0416 from time 
% which implies it is 1-consistent when the predictions are precise, i.e. $\X = \Xpred$. 
% % $0$ to time $t_n$ and 
% The server makes adjustments if needed (i.e.,  $p_i \neq \hat p_i$) before and when the last request arrives. 
% % Then, 
% Finally, at time $t_n$, it decides to continue on the current route or not. Therefore, we
% % distinguish between 
% discuss the following two cases depending on the relationship of $r_1$ and $r_2$. Note that $t_n \leq \costopt$ and 
% %0420 $L_{off}(U) \leq \costopt$ for any request subset $U$.
% $|T_{U_{t}}| \leq Z^{OPT}$ for any $t$.
% \begin{itemize}
%     \item{1. $r_1 \leq r_2$.} In this case, the server knows that continuing on the route $\hatT$ takes less time than redesigning a new one, which implies the errors are small. Thus, it follows the route $\hat T$ from beginning to end. By Theorem~\ref{thm:naive}, the completion time of the algorithm can be bounded by $\costalg \leq \costopt + 2 \errortime + 4 \errorpos$.
%     \item{2. $r_1 > r_2$.} In this case, it is better to go back to the origin and design a new route. The server arrives the origin $o$ at time $t_n + d(p(t_n), o)$ and starts to follow a new route $T$, which visits all unserved requests in $U$. Because there is no request arrives after $t_n$, the server completes all of the requests at time $\costalg = t_n + d(p(t_n), o) + |T_{U_{t_n}}|$. In addition, since the server moves with unit speed, we know the distance it can travel between time $0$ and time $t_n$ is bounded by $d(p(t_n), o) \leq t_n$. Combining with the two trivial inequalities mentioned above, we obtain the result $\costalg \leq 3 \costopt$.
% \end{itemize}
% As the server choose the fastest route among the two possible options, the competitive ratio can be stated as $\min \{3, 1+(2 \errortime + 4 \errorpos) / \costopt\}$.
% \end{proof}

\begin{restatable}{rCor}{corLASw}\label{cor:LASw}
The~\algI~algorithm is a $\min \{3.5, 2.5 + (3.5 \errortime + 7 \errorpos) / \costopt\}$-competitive polynomial-time algorithm using Christofides' 
%%shou algorithm.
heuristic. 
\end{restatable}
%\subsection{A Special Case}




==> Online TSP with Predictions_v1r/sec_4_a_single_request.tex <==
\section{Predict the Last Arrival Time}\label{sec:4} 
%%shou By carefully examining the \PAH~algorithm, we 
One can 
observe that Corollary~\ref{cor:PAHwait} provides 
%%shou an 
a special 
insight about 
%%shou designing algorithms; 
predictions. 
That is, when the last request arrives, 
%%shou
if the server is at the origin,  
we can apply an offline algorithm 
%%shou of 
for the 
TSP to 
%%shou solve 
serve all 
the remaining unserved requests without dealing with the release time of the requests. Based on the %%shou above 
insight, 
it is fair to consider 
%%shou the other 
another 
simpler model by predicting the arrival time of the last requests $\hat{t}_n$ only, 
%%shou 
rather than 
%%shou instead of 
predicting a whole sequence of future requests.  
%%
%We consider the model 1 by giving the arrival time of the last request $\hat t_{last}$ as our prediction. 
%%shou However, since we only obtain a limited information for a single point, 
%%shou
Though 
we first show 
%%shou that 
the restricted power of the model 
%%shou
due to the limited information of predictions. Next, 
%%shou QQQ
compared to \PAH, 
we introduce a 
%%0422 new 
pure online algorithm, \redesign, 
%0406 \textsc{Simpler-Plan-At-Home}(SPAH) which is exactly a simpler version of the PAH algorithm. 
%%shou Finally, we give 
and present 
a polynomial-time learning-augmented algorithm 
%%shou that combines the prediction $\hat t_n$ and the pure online algorithm.
for the restricted prediction model. 


%%shou We first show that such prediction cannot break the lower bound . 
Intuitively, 
%%shou
if the arrival time of the last request is given, 
%%shou
the server can just wait until the last request 
%%shou comes
arrives before starting a route. 
%%shou In this case, 
That is, 
the completion time is $\costalg \leq t_n + |T_{\X}| \leq 2 \costopt$.
%%shou Specifically, 
Precisely, 
%%shou even when the server has 
%%shou the 
%%shou additional information,
even when the prediction is correct, 
%%shou QQQ 
the lower bound of 2, i.e., 
%%shou the proof of 
Theorem 3.2 in~\cite{ausiello2001algorithms} still holds and so does the 
%%shou result.
corollary. 


\begin{theorem}[\cite{ausiello2001algorithms}, Theorem 3.2]\label{thm:PAHlb}
There is no $c$-competitive algorithm for the OLTSP with $c < 2$.
\end{theorem}

\begin{restatable}{rCor}{corlblast}\label{thm:>2}
Given the arrival time of the last request $\hat t_n$, 
%%shou as the prediction, 
there is no $c$-competitive algorithm with $c < 2$.
\end{restatable}


\begin{comment}
\begin{psketch}
%0419 Assume the number of requests $n$ is given. 
\end{psketch}
\end{comment}

%0406
\begin{comment}
\begin{proof}
%0406 We omit the proof here due to the page limit and present the details in the Appendix.
We consider the perfect prediction $\hatt_n = t_n$.
\end{proof}
\end{comment}

%%shou
In order to design a learning-augmented online algorithm with robustness, we
%%shou discuss 
present 
a simpler online algorithm, \redesign, 
%%shou which is simpler 
than \PAH, 
%%shou ~algorithm but 
and it can
achieve the same competitive ratio of $3$ in polynomial time. 
%%shou
Compared to \PAH, 
the~\redesign~algorithm always goes back to the origin and redesign an optimal (or approximate) route for $U_t$, 
whenever a new request $x_i$ arrives. 
The following two lemmas show that the~\redesign~algorithm is $3$-competitive. 

%%shou
\begin{comment}
As in \PAH, a server operated by the~\redesign~algorithm starts to follow an approximate route $T_{U_t}$ for released unserved requests when the server is at the origin, i.e., $p(t) = o$. However, we remove the distance condition in the sense that the server goes back to the origin whenever a new request $x_i$ arrives. 
%0403 Namely, the behavior of the server depends only on whether it is at the origin or not. 
We prove the following two lemmas to show that the~\redesign~algorithm is $3$-competitive:
\end{comment}

\begin{comment}
\begin{algorithm}
    \caption{A Pure Online Algorithm}\label{alg:metric3}
    \begin{algorithmic}[1] %1: provides the line numbered at every line
    \State \textbf{If} the server is at the origin $o$ \textbf{then}
        \State \quad Start to follow a route $T$ which visits all unserved requests and returns to the origin $o$.
    \State \textbf{ElseIf} the server is currently following a route $T'$ \textbf{then}
        \State \quad \textbf{If} a new request $x_i = (t_i, p_i)$ arrives \textbf{then}
            \State \quad \quad Interrupt route $T'$ and go back to the origin along the shortest path.
        \State \quad \textbf{Else}
            \State \quad \quad Continue on the current route $T'$.
        %0403
        \State \quad \textbf{EndIf}
    %0403
    \State \textbf{EndIf}
    \end{algorithmic}
\end{algorithm}
\end{comment}

\begin{algorithm}
    \caption{\redesign 
    % Algorithm
    }\label{alg:replan}
    
    \begin{algorithmic}[1] %1: provides the line numbered at every line
    % \Procedure{Replan}{The set of current released unserved requests $U_t$}
    \Require The current time $t$ and the set of current released unserved requests $U_t$
    \State \textbf{While} $U_t \neq \emptyset$ \textbf{do}
        \State \quad \textbf{If} the server is at the origin $o$ \textbf{then}
            \State \quad \quad Start to follow a route $T_{U_t}$ to serve the requests in $U_t$ and return to the origin $o$.
        \State \quad \textbf{ElseIf} the server is 
        %0420 on
        currently moving along
        a route $T_{U_{t'}}$, for some $t' < t$ \textbf{then}
            \State \quad \quad \textbf{If} a new request $x_i = (t_i, p_i)$ arrives \textbf{then}
            %0406 \State \quad Interrupt route $T'$
                \State \quad \quad \quad Go back to the origin $o$.
            \State \quad \quad \textbf{EndIf}
            %0406 along the shortest path.
        \State \quad \textbf{EndIf}
    % \EndProcedure
    \State \textbf{EndWhile}
    \end{algorithmic}
\end{algorithm}

\begin{restatable}{rLem}{lemhalf}\label{lem:1/2}
Given 
%%shou
that $p(t)$ is the current position of a server 
operated by the~\redesign~algorithm, we have $d(p(t), o) \leq \frac{1}{2} \costopt$, for any $t$.
\end{restatable}
% \begin{proof}
% A simple explanation is that 
% (1) at any time $t$ during the execution of the algorithm, the distance between the online server and the origin $d(p(t), o)$ is at most the length between the farthest request and the origin, and 
% (2) the offline route must be longer than twice the distance from the farthest request to the origin.
% Now, we prove the lemma in a more rigorous way by specifying the state of the server at time $t$.

% \begin{itemize}
%     \item {1. The server is at the origin $o$ at time $t$.} Trivially, we get $d(p(t), o) = 0 \leq \frac{1}{2} \costopt$.
%     \item {2. The server is not at the origin $o$ at time $t$.} 
%     %0403 We need an upper bound on $d(p(t), o)$ for this case, and 
%     In this case, we know that the server is either on a route $T_{U_{t'}}$ found by Christofides' algorithm, where $t' < t$, or already on its way home due to the arrival of some earlier request. 
%     %0403 Let $U$ be the set of requests the server plans to visit on a route $T$, which is designed when the server is at the origin, and let $T^*$ denote an optimal route to visit requests in $U$. 
%     Let $T^*$ denote an optimal route to visit the set of requests for which the route $T_{U_{t'}}$ is planned.
%     Note that neither route $T_{U_{t'}}$ nor route $T^*$ considers the release time of the requests.
%     \begin{itemize}
%         \item {2-1. The server is on the route $T_{U_{t'}}$.} This implies that the server is traveling between a pair of points, denoted as $a$ and $b$, where a point must be the position of a request $x_i$ or the origin $o$. Since route $T^*$ contains at least point $a$, point $b$, and the origin $o$, we know $|T^*| \geq d(o, a) + d(a, b) + d(b, o)$. Then, we have $d(p(t), o) \leq \min \{ d(p(t), a) + d(a, o), d(p(t),b) + d(b, o)\} \leq \frac{1}{2} |T^*| \leq \frac{1}{2} \costopt$. 
%         \item {2-2. The server is on its way back home.} 
%         This implies that the server has terminated a route $T_{U_{t'}}$.
%         We know that some request $x_i=(t_i, p_i)$ arrives between the time $t'$
%         %0420 when the route $T_{U_{t'}}$ starts 
%         and time $t$. 
%         %0420 Thus, the server has terminated the route $T_{U_{t'}}$.
%         As we can obtain $d(p(t_i), o) \leq \frac{1}{2} \costopt$ by the above argument, we know also $d(p(t), o) \leq d(p(t_i), o) \leq \frac{1}{2} \costopt$.
%     \end{itemize}
% \end{itemize}
% \end{proof}

\begin{restatable}{rLem}{lemreplan}\label{lem:replan}
The~\redesign~algorithm is
% \ref{alg:replan} 
a $3$-competitive polynomial-time algorithm for the OLTSP in a metric space using Christofides' %%shou algorithm.
heuristic. 
\end{restatable}
% \begin{proof}
% %0420 Let $S_t$ be the set of requests that are served before time $t$.
% %0403 Since the server goes back to the origin whenever a request arrives, 
% Note that the algorithm completes when the server receives the last request $x_n$, goes back to the origin $o$, and follows the last route $T_{U_{t_n}}$ found by Christofides' algorithm.
% Namely, the completion time is $\costalg = t_n + d(p(t_n), o) + |T_{U_{t_n}}|$.
% By the two natural bounds $t_n \leq \costopt$ and $|T_{U_{t_n}}| \leq 1.5 \costopt$, we know the completion time is bounded by $\costalg \leq 2.5 \costopt + d(p(t_n), o)$. Meanwhile, we have $d(p(t_n), o) \leq 0.5 \costopt$ by Lemma~\ref{lem:1/2}. Combining them, we get $\costalg \leq 3 \costopt$.
% \end{proof}

\subsection{The Algorithm}\label{sec:4-1}
In this section, we present the~\algL~algorithm and show that it is $\min \{4, 2.5 + |\errorlast| / \costopt \}$-competitive. The idea of the algorithm is to ensure the server 
%%shou is 
to arrive 
at the origin $o$ at time $\hatt_n$ and follow the~\redesign~algorithm,  
%%shou pure online algorithm, , 
for the rest of the 
%%shou time. 
execution. 

It is motivated by the desire to 
%%shou make sure 
enable 
the server 
%%shou is close to 
to approach
the origin at time $t_n$, when the last request arrives.
An intuitive strategy is to wait at the origin $o$ until the predicted last arrival time $\hat t_n$ and then follow a route $T_{U_{\hat t_n}}$ that serves whatever is in hands. It seems to beat the previous result easily when the prediction is perfectly accurate, i.e., $\hat t_n = t_n$. However, waiting at the origin is potentially costly when the quality of predictions is undisclosed. If the expected time $\hat t_n$ is too late, the server might postpone serving requests for a long time. 
In consequence, the competitive ratio might extend to infinity 
%%shou and 
so that 
the algorithm has no robustness. 
%%shou That is why we need the pure online algorithm.

We propose a learning-augmented algorithm, 
called~\algL.
%%shou and formally describe it in . 
Basically, 
we incorporate the predicted time $\hat t_n$ into the~\redesign~algorithm by forcing the server to return 
%%shou back 
to the origin at time $\hatt_n$ in order to hedge against the possible loss.
At any time $t$, if the server is at the origin $o$, it finds an approximate route $T_{U_t}$ to visit all released unserved requests in $U_t$ by using Christofides' 
%%shou algorithm. 
heuristic. 
%The server knows it will return to the origin at time $t+|T_{U_t}|$ if the route is not interrupted. 
%%shou As in 
Similar to~\algNI, we add a gadget here: if the route is too long (i.e., $t < \hat t_n < t+|T_{U_t}|$), the server should find the moment $t_{back}$ to stop the route $T_{U_t}$ and start moving towards the origin 
%%shou $o$ 
so that the server can arrive 
%%shou
at the origin 
%%shou
exactly at time $\hat t_n$. 
On the other hand, if the server is 
%%shou following 
moving along 
a route $T_{U_{t'}}$ and a new request $x_i$ arrives,
%0403 at time $t_i$ at position $p_i$
the server goes back to the origin $o$ immediately at time $t_i$, as~\redesign~performs.

\begin{algorithm}
    % \caption{An Algorithm with Prediction of the Last ArrivalTime}
    \caption{\textsc{Learning-Augmented Routing With Last Arrival
    Time (LAR-LAST)}}\label{alg:LAM}
    \begin{algorithmic}[1] %1: provides the line numbered at every line
    \Require The current time $t$, the predicted last arrival time $\hat t_n$, and the set of current released unserved requests $U_t$.
    \State \textbf{While} $U_t \neq \emptyset$ \textbf{do}
    \State \quad \textbf{If} the server is at the origin $o$ (i.e., $p(t) = o$) \textbf{then}
        \State \quad \quad Compute an approximate route $T_{U_{t}}$ to serve all the requests in $U_t$ and return to the  
        \Statex \quad \quad origin $o$;
        \State \quad \quad \textbf{If} $t < \hat t_n$ and $t + |T_{U_{t}}| > \hat t_n$ \textbf{then}
        \Comment{Add a gadget}
            \State \quad \quad \quad Find 
            %0420 a time 
            the moment $t_{back}$ such that $t_{back} + d(p(t_{back}), o) = \hat t_n$;
            \State \quad \quad \quad Redesign a route $T'_{U_{t}}$ by asking the the server to go back to the origin $o$ at time
            \Statex \quad \quad \quad $t_{back}$ along the shortest path;
            \State \quad \quad \quad Start to follow the route $T'_{U_{t}}$.
        \State \quad \quad \textbf{Else}
            \State \quad \quad \quad Start to follow the route $T_{U_{t}}$.
        %0403
        \State \quad \quad \textbf{EndIf}
    \State \quad \textbf{ElseIf} the server is currently 
    %0420 following 
    moving along a route $T_{U_{t'}}$, for some $t' < t$ \textbf{then}
        \State \quad \quad \textbf{If} a new request $x_i = (t_i, p_i)$ arrives \textbf{then}
        \Comment{Similar to \redesign}
            \State \quad \quad \quad Go back to the origin $o$.
            %along the shortest path.
        %0403
        \State \quad \quad \textbf{EndIf}
    %0403
    \State \quad \textbf{EndIf}
    \State \textbf{EndWhile}
    \end{algorithmic}
\end{algorithm}

%0403 To analyze the performance of Algorithm~\algL, we first show the existence of the $t_{back}$.
%0420 Next, we show the existence of the $t_{back}$ before proving the main result of Algorithm~\algL.
Next, we prove the main result of the~\algL~algorithm. Note that the existence of $t_{back}$ can be %%shou
similarly 
derived from Lemma~\ref{lem:tback}.


\begin{restatable}{rThm}{thmLAM}\label{thm:LAM}
The~\algL~algorithm is a $\min \{ 4, 2.5 + |\errorlast| / \costopt \}$-competitive polynomial-time algorithm,
%0403 The competitive ratio of Algorithm~\algL is $\min \{ 4, 2.5 + |\errorlast| / \costopt \}$, 
where $\errorlast = \hat t_n - t_n$. Therefore, the~\algL~algorithm is $2.5$-consistent, $4$-robust and $|\errorlast|$-smooth.
\end{restatable}
% \begin{proof}
% The most important thing is the server's position when the last request $x_n$ arrives, and the ideal situation is that the server is at the origin $o$ at time $t_n$, i.e., $p(t_n) = o$. We distinguish between two main cases depending on the relationship between the predicted and actual last arrival time, $\hat t_n$ and $t_n$. 
% %0420 Let $S_{\leq \hat t_n}$ (resp. $S_{\leq t_n}$) be the set of requests which are served before $\hat t_n$ (resp. $t_n$). 
% Note that we get $t_n \leq \costopt$ and $|T_{U_t}| \leq 1.5 \costopt$ for any $t$ trivially.

% \begin{itemize}
%     \item {1. $\hat t_n \leq t_n$.} The server is at the origin $o$ at time $\hatt_n$. After then, it receives some request and returns to the origin only when a request arrives or a route is completed. Therefore, the completion time is $\costalg = t_n + d(p(t_n), o) + |T_{U_{t_n}}|$. By the above two inequalities, this leaves us $\costalg \leq 2.5 \costopt + d(p(t_n), o)$ to discuss.
%         \begin{itemize}
%             \item {1-1.} By Lemma~\ref{lem:1/2}, the distance from the server to the origin is bounded at any moment. We get $d(p(t_n), o) \leq 0.5 \costopt$ and our first bound $\costalg \leq 3 \costopt$. 
%             \item {1-2.} Although the server might have left the origin at time $t_n$, it cannot be too far if the error $|\errorlast|$ is small. Seeing that the server moves with unit speed, the distance it can travel between time $\hat t_n$ and $t_n$ is at most $t_n - \hat t_n$. As the server is at the origin $o$ at time $\hat t_n$, we obtain $d(p(t_n), o) \leq t_n - \hat t_n = - \errorlast$. Thus, our second bound for case 1 is $\costalg \leq 2.5 \costopt + (- \errorlast)$, where $\errorlast \leq 0$.
%         \end{itemize}
%     \item {2. $\hat t_n > t_n$.} 
%     Since no request arrives after time $\hat t_n$ and the server could start its last route $T_{U_{\hat t_n}}$ at $\hat t_n$ (if needed), we have $\costalg \leq \hatt_n + |T_{U_{\hat t_n}}|$.
%     Let $t_L$ be the last time before $\hat t_n$ that a route is planned and $T^L$ be the original route planned at time $t_L$. Let $T'^L$ be the new route if $T^L$ is adjusted and equal to $T^L$ if not. Note that $t_L + |T'^L| \leq \hat t_n$ due to the choice of $t_{back}$.
%         \begin{itemize}
%             \item {2-1. $t_L + |T^L| \leq \hat t_n$.} The server finishes serving all requests in $\X$ before time $\hat t_n$ and thus $\costalg \leq \hatt_n$. Note that none of the routes the server has followed is too long and needs to be adjusted. In this case, since the algorithm runs in the same way as the~\redesign~algorithm, we know that $\costalg \leq 3 \costopt$ still holds by Lemma~\ref{lem:replan}.
%             \item {2-2. $t_L + |T^L| > \hat t_n$ and $t_n \leq t_L$.} The route $T^L$ is too long, and the algorithm find a time $t_{back}$ and a substitute route $T'^L$ so that the server can be at the origin $o$ at time $\hat t_n$. Since every request in $\X$ has arrived before $t_L$, the server could have finished visiting all requests by following the original route $T^L$. However, the server chooses the adjusted route $T'^L$ instead. The additional cost of moving back to the origin is at most $2 d(p(t_{back}), o)$. Thus, by Lemma~\ref{lem:1/2} and Lemma~\ref{lem:replan}, the completion time is $\costalg \leq 3 \costopt + 2 d(p(t_{back}), o) \leq 4 \costopt$.
%             \item {2-3. $t_L + |T^L| > \hat t_n$ and $t_n > t_L$.} Again, the route $T^L$ is too long, and at least one request is unknown at time $t_L$.
%             Also, the server cannot visit all requests in $\X$ before $\hat t_n$ and has to start a new route at that moment, which is the last route since all requests have arrived by then.  Noting the route $T'^L$ also satisfies $|T'^L| \leq 1.5 \costopt$, the completion time is 
%             \begin{align*}
%                 \costalg &\leq \hatt_n + |T_{U_{\hat t_n}}|
%                 \\& = t_L + |T'^L| + |T_{U_{\hat t_n}}|
%                 \\& \leq t_n + |T'^L| + |T_{U_{\hat t_n}}|
%                 \\& \leq 4 \costopt
%             \end{align*}
%             Combining with the results in 2-1 and 2-2, we have our first bound $\costalg \leq 4  \costopt$.
%             \item {2-4.} If the error $|\errorlast|$ is not zero, the server might have not reached the origin at time $t_n$. However, if the error is small, it must be close to the origin since it has planned to reach there at time $\hat t_n$. 
%             %0403 Note that $\hat{t}_{max} = t_{max} + \varepsilon^t_{max}$. 
%             Formally, we have $\costalg \leq t_n + \errorlast + |T_{U_{\hat t_n}}|$ by replacing $\hatt_n$ with $t_n + \errorlast$, which leads to our second bound $\costalg \leq 2.5 \costopt + \errorlast$.
%             %0403 \begin{align*}
%                 %0403 \costalg &\leq t_n + \errorlast + L_{Chr}(\X \backslash S_{\leq \hat t_{last}})\\ & \leq \costopt + \errorlast + 1.5 \costopt\\& \leq 2.5 \costopt + \errorlast
%             %0403 \end{align*}
%         \end{itemize}
% \end{itemize}

% Both cases show $\costalg \leq \min \{4 \costopt, 2.5 \costopt + |\errorlast|\}$, which completes the proof.
% \end{proof}

==> Online TSP with Predictions_v1r/sec_5_ride_a_dial.tex <==
\section{Extension to The Dial-a-Ride Problem}
%0416After studying the OLDARP, 
As we found the OLDARP has some properties similar to the OLTSP, we extend our models and algorithms to the dial-a-ride problem with unlimited capacity. 
%0420 \subsection{Learning-Augmented Algorithms}
%0420 Here, we discuss how our algorithms can be extended to the OLDARP. 
We only mention the necessary changes for adapting the proposed algorithms to this problem as well as the results we obtain, and the details are presented in the Appendix~\ref{LADARP}. The main difference is that the learning-augmented algorithms for the OLDARP are based on the~\redesign~algorithm,
%: whenever a new request 
%0420 $x_i = (t_i, a_i, b_i)$ 
%arrives, the server goes back to the origin and follows a route that visits all of the released unserved requests. 
%This strategy 
which yields a competitive ratio of $2.5$ when ignoring the computational issue. Note that although the \algsmartstart~algorithm~\cite{ascheuer2000online} has a better competitive ratio than the \redesign~strategy,
%0406 is $2$-competitive, 
it is also more complicated and thus more difficult to be integrated with predictions.

First, we 
%0420 modify 
develop the~\algdarNI~algorithm by 
substituting the \redesign~strategy for the \PAH~algorithm in~\algNI. 
%0420If any request $x_i$ arrives after $\lambda |\hat T|$, the server starts the route $\hat T$ at time $t_i$. 
%Unless the server is following the predicted route $\hat T$, the server goes back to the origin whenever a new request arrives, regardless of the request's position. 
Note that if the server 
%stops following a route and 
gets to go back to the origin when carrying some requests, it brings all of them to the origin. This algorithm is $(1.5+ \lambda)$-consistent and $(3.5 + 2.5 / \lambda)$-robust but not smooth.
%
Next, we consider the~\algdarI~algorithm. 
%The only thing we need to clarify here is how the server adjusts the route when a request is released. 
Note that a route for the OLDARP can be described as a series of pickup and delivery positions instead of requests. 
%0420 When a request arrives, the server adds the position $a_i$ (resp. $b_i$) after the predicted one $\hat a_i$ (resp. $\hat b_i$). 
Accordingly, when a request becomes known, the server needs to update two positions.
Then, the algorithm is 
%0406 $\min \{3, 1 + 2 (\errortime + \errorpos) / \costopt\}$-competitive, which means it is 
$1$-consistent, $3$-robust, and $(2 \errortime + 4 \errorpos)$-smooth.
%
Last, we use the~\algdarL~algorithm for the prediction of last arrival time, which replaces Christofides' heuristic with the optimal solutions
%0420algorithm 
for the offline DARP without release time. This change makes the algorithm
%0406 $\min\{3.5, 2 + |\errorlast| / \costopt\}$-competitive, which means it is 
$2$-consistent, $3.5$-robust, and $|\errorlast|$-smooth.

==> Online TSP with Predictions_v1r/sec_6_conclusion.tex <==
\section{Conclusion}
%%shou
In this study, we have investigated 
%%shou the study of 
two well-known online routing problems 
based on the learning-augmented framework. 
%%
The proposed prediction models and results raise some interesting 
questions to further explore. First, it 
%%shou
would be of interest to improve the current 
%%shou
competitive results;  
especially coping with waiting strategies is usually helpful to 
%%shou the performance. 
the OLTSP and the OLDARP. 
% Note that the algorithm in our last model does not perform better than the current best algorithm \algsmartstart, which is $2$-competitive. We observe that \algsmartstart~achieves a better result than the \replan~and \textsc{Ignore} algorithms by using the waiting strategy. 
Note that the currently best results for 
%%shou many variants of the online routing problems 
these two problems
exploited waiting strategies, which leaves us an open problem to 
improve our learning-augmented online algorithms by incorporating a waiting strategy.
%%shou
It would be also worthwhile to design learning-augmented online algorithms for other variants of online routing problems 
%%shou such as 
with
limited capacity or 
%%shou restricted total serving number.
multiple servers. 
% Furthermore, we would also like to discuss the DARP with limited capacity.
